Activate Me!: Designing Efficient Activation Functions for Privacy-Preserving Machine Learning with Fully Homomorphic Encryption

The growing adoption of machine learning in sensitive areas such as healthcare and defense introduces significant privacy and security challenges. These domains demand robust data protection, as models depend on large volumes of sensitive information for both training and inference. Fully Homomorphic Encryption (FHE) presents a compelling solution by enabling computations directly on encrypted data, maintaining confidentiality across the entire machine learning workflow. However, FHE inherently supports only linear operations, making it difficult to implement non-linear activation functions, essential components of modern neural networks. This work focuses on designing, implementing, and evaluating activation functions tailored for FHE-based machine learning. We investigate two commonly used functions: the Square function and Rectified Linear Unit (ReLU), using LeNet-5 and ResNet-20 architectures with the CKKS scheme from the OpenFHE library. For ReLU, we assess two methods: a conventional low-degree polynomial approximation and a novel scheme-switching technique that securely evaluates ReLU under FHE constraints. Our findings show that the Square function performs well in shallow networks like LeNet-5, achieving 99.4% accuracy with 128 seconds per image. In contrast, deeper models like ResNet-20 benefit more from ReLU. The polynomial approximation yields 83.8% accuracy with 1,145 seconds per image, while our scheme-switching method improves accuracy to 89.8%, albeit with a longer inference time of 1,697 seconds. These results underscore a critical trade-off in FHE-based ML: faster activation functions often reduce accuracy, whereas those preserving accuracy demand greater computational resources.

==> Makefile <==
# Add a list of home-made EPS figures here.
PDFFIGURES=figs/arch_pipeline.pdf figs/arch_icswitch.pdf

.SUFFIXES: .fig .eps .ps .dvi .bbl .bib .tex .pdf

FIGURES=${wildcard *.fig}
EPSFIGFILES=${FIGURES:.fig=.eps}
TEXFILES=*.tex

all: pdf   

force: rmdone all

dvi: paper.dvi

xdvi: paper.dvi
	xdvi paper.dvi

gv: paper.ps
	gv paper.ps

ps: paper.ps 

pdf: paper.pdf

rmdone:
	rm -f done.flag

done.flag:
	touch done.flag

printerrors:
	@echo "*****************************"; \
	echo Overview of typeset warnings: ; \
        echo "****************************"; \
	grep "Underfull" paper.log; \
	grep "Overfull" paper.log; \
	echo ; \
        echo "***************************"; \
	echo Overview of latex warnings: ; \
        echo "***************************"; \
	grep "LaTeX Warning" paper.log; \
        echo "***************************"; \
	echo ; \
        echo "***************************"; \
	echo Overview of bibtex warnings: ; \
        echo "***************************"; \
        grep ^Warning-- paper.blg; \
	echo "***************************"; \
	echo ; \
        echo "*************************"; \
	echo Overview of latex errors: ; \
        echo "*************************"; \
	grep "^!" paper.log; \
        echo "*************************"; \
	echo

paper.bbl: paper.bib $(TEXFILES) Makefile done.flag
	pdflatex -interaction=batchmode paper.tex || true
	rm -f $*.pdf
	bibtex -terse $*

paper.pdf: $(TEXFILES) $(PDFFIGFILES) paper.bbl Makefile done.flag
	@echo Running latex once.; \
	while ( pdflatex -interaction=nonstopmode paper.tex; grep Rerun paper.log ) ; do \
          echo; \
          echo "*********************************"; \
          echo "*********************************"; \
          echo Reruning to complete compilation.; \
          echo "*********************************"; \
          echo "*********************************"; \
	done; \
        echo "***************************"; \
	echo DVI file generated.; \
        echo "***************************"; \
	echo ; \
	make printerrors 
			
clean:
	rm -f *.lof *.lot *.pfg *~ *.aux *.dvi *.blg *.log *.bbl $(EPSFIGFILES) *.bak paper.ps paper.pdf *.toc *.swp done.flag




==> sections/architectures.tex <==

\begin{table*}[ht]
    \centering
    \caption{Breakdown of layers in the selected neural network architectures.}
    \begin{tabularx}{\textwidth}{|l|X|X|X|X|}
    \hline
    \centering \textbf{Architecture} & \centering \textbf{Convolution Layers} & \centering \textbf{Average Pooling Layers} & \centering \textbf{Fully Connected Layers} & \centering \arraybackslash \textbf{ReLU Activations} \\
    \hline
    LeNet-5 & 2 & 2 & 3 & 4 \\
    \hline
    AlexNet & 5 & 3 & 3 & 7 \\
    \hline
    VGG-11 & 8 & 5 & 3 & 10 \\
    \hline
    VGG-16 & 13 & 5 & 3 & 15 \\
    \hline
    ResNet-20 & 22 & 1 & 1 & 22 \\
    \hline
    ResNet-34 & 37 & 1 & 1 & 37 \\
    \hline
    \end{tabularx}
    \label{table:arch_breakdown}
\end{table*}

